Duality for Optimal Multi-Item, Multi-Bidder Auction Design: Revenue Certificates through Deep Learning

Characterizing revenue-optimal auctions for multi-item, multi-bidder settings remains a fundamental open problem, with no known closed-form solution existing beyond restrictive binary-type instances. This has motivated interest in computational approaches to optimal auction design. In this paper, we introduce the first computational framework that directly tackles the dual problem for multi-item, multi-bidder auctions and dominant-strategy incentive compatibility (DSIC), generating certified revenue upper bounds. Our approach parametrizes Lagrange multipliers with a structurally guaranteed strict flow-conservation property using neural networks, enabling efficient optimization over feasible dual solutions via gradient descent. To bridge the gap between discrete computational methods and theoretical guarantees for continuous types, we develop a novel lifting technique that maps dual certificates from coarse discretizations to fine refinements. We prove that lifting gives valid revenue upper bounds for multi-item, multi-bidder auctions with continuous uniform valuations. Furthermore, we give a generalized lifting construction for arbitrary continuous distributions and demonstrate that these lifted duals converge to the revenue of the original continuous problem in the discrete limit. We validate this computational framework for the dual auction design problem by recovering known analytical mechanisms for canonical instances. For multi-item multi-bidder problems, our framework establishes a small gap between the optimal revenue and best-known DSIC mechanisms, providing computational certificates of near-optimality.

==> backup.tex <==





\subsection{Convergence to the continuous revenue}

DSIC: for every bidder $i$, for all $v_i\in[0,H]^m$, all reports
$v_i'\in[0,H]^m\cup\{\varnothing\}$, and 
almost every 
$v_{-i}$,
\begin{equation}\label{eq:DSIC-cont}
\sum_{j=1}^m x_{ij}(v_i,v_{-i})\,v_{ij}-p_i(v_i,v_{-i})
\;\ge\;
\sum_{j=1}^m x_{ij}(v_i',v_{-i})\,v_{ij}-p_i(v_i',v_{-i}).
\end{equation}
The expected revenue is
\[
\Rev^{(x,p)}(D):=\int_V f(v)\Big(\sum_{i=1}^n p_i(v)\Big)\,\dV,
\qquad
\Rev(D):=\sup_{(x,p)\ \text{DSIC/IR feasible}}\Rev^{(x,p)}(D).
\]


In a discrete problem, dual variables $\lambda_i^{v_{-i}}(v_i,v_i')$ are Lagrange
multipliers attached to each DSIC constraint. In continuous type spaces we
model them as \emph{kernels / measures}.

\paragraph{Dual object (kernel form).}
Fix $i\in[n]$. For almost every $v_{-i}$, let
\[
\lambda_i^{v_{-i}}:\ [0,H]^m\times \mathcal{B}([0,H]^m\cup\{\varnothing\})\to [0,\infty]
\]
be a nonnegative kernel, so that for each $v_i$,
$A\mapsto \lambda_i^{v_{-i}}(v_i,A)$ is a finite measure on
$[0,H]^m\cup\{\varnothing\}$, and for each measurable $A$,
$v_i\mapsto \lambda_i^{v_{-i}}(v_i,A)$ is measurable.

\paragraph{Flow conservation.}
We say $\lambda$ \emph{conserves flow} if for every bidder $i$ and almost every
$v_{-i}$, for almost every $v_i$,
\begin{equation}\label{eq:flow-cont}
\lambda_i^{v_{-i}}(v_i,[0,H]^m\cup\{\varnothing\})
\;=\;
f(v_i,v_{-i}) \;+\; \int_{[0,H]^m}\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i) \mathrm{d}u_i.
\end{equation}


\paragraph{Virtual values.}
Given any flow-conserving $\lambda$, define (for almost every $v$ with $f(v)>0$)
\begin{equation}\label{eq:virt-cont}
\Phi_{ij}^{\lambda}(v)
\;:=\;
v_{ij}
\;-\;
\frac{1}{f(v)}
\int_{[0,H]^m} (u_{ij}-v_{ij})\,\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i).
\end{equation}


\begin{lemma}[Continuous Weak Duality)]\label{lem:cont-thm24}
Assume $\lambda$ conserves flow in the sense of \cref{eq:flow-cont}.
Then for every DSIC/IR feasible mechanism $(x,p)$,
\begin{equation}\label{eq:cont-thm24}
\int_V f(v)\Big(\sum_{i=1}^n p_i(v)\Big)\,\dV
\;\le\;
\int_V f(v)\Big(\sum_{i=1}^n\sum_{j=1}^m x_{ij}(v)\,\Phi_{ij}^\lambda(v)\Big)\,\dV.
\end{equation}
Consequently,
\[
\Rev(D)\;\le\;
\sup_{x\ \text{feasible}}\int_V f(v)\Big(\sum_{i,j}x_{ij}(v)\Phi_{ij}^\lambda(v)\Big)\,\dV
\;=\;
\int_V f(v)\Big(\sum_{j=1}^m \max_{i\in[n]}(\Phi_{ij}^\lambda(v))_+\Big)\,\dV.
\]
\end{lemma}

\begin{proof}
Fix a DSIC/IR feasible $(x,p)$. Define the (ex post) utility
\[
U_i(v_i;v_{-i}) := \sum_{j=1}^m x_{ij}(v_i,v_{-i})\,v_{ij}-p_i(v_i,v_{-i}).
\]
DSIC in \cref{eq:DSIC-cont} says that for every $i$, almost every $v_{-i}$,
every $v_i\in[0,H]^m$, and every report $v_i'\in[0,H]^m\cup\{\varnothing\}$,
\[
U_i(v_i;v_{-i}) \;\ge\; \sum_{j=1}^m x_{ij}(v_i',v_{-i})\,v_{ij}-p_i(v_i',v_{-i}).
\]
Rearranging,
\begin{equation}\label{eq:DSIC-rearr}
\sum_{j=1}^m v_{ij}\big(x_{ij}(v_i,v_{-i})-x_{ij}(v_i',v_{-i})\big)
\;-\;
\big(p_i(v_i,v_{-i})-p_i(v_i',v_{-i})\big)
\;\ge\;0.
\end{equation}
Multiply \cref{eq:DSIC-rearr} by the nonnegative measure
$\lambda_i^{v_{-i}}(v_i,\mathrm{d}v_i')$ and integrate in $v_i'$.
Since the integrand is nonnegative, Tonelli's theorem applies and yields, for
each $i$ and almost every $v_{-i}$ and every $v_i$,
\begin{align}
0
&\le
\int_{[0,H]^m\cup\{\varnothing\}}
\Bigg[
\sum_{j=1}^m v_{ij}\big(x_{ij}(v_i,v_{-i})-x_{ij}(v_i',v_{-i})\big)
-\big(p_i(v_i,v_{-i})-p_i(v_i',v_{-i})\big)
\Bigg]\,
\lambda_i^{v_{-i}}(v_i,\mathrm{d}v_i').
\label{eq:integrated-dsic}
\end{align}
Now integrate \cref{eq:integrated-dsic} over $v_i$ and $v_{-i}$ (again Tonelli
applies, since all terms are integrable on the bounded support, and $\lambda$
is finite by assumption):
\begin{align}
0
&\le
\int_{V_{-i}}\int_{V_i}
\int_{[0,H]^m\cup\{\varnothing\}}
\Bigg[
\sum_{j=1}^m v_{ij}\big(x_{ij}(v_i,v_{-i})-x_{ij}(v_i',v_{-i})\big)
-\big(p_i(v_i,v_{-i})-p_i(v_i',v_{-i})\big)
\Bigg]\,
\lambda_i^{v_{-i}}(v_i,\mathrm{d}v_i')\,\mathrm{d}v_i\,\mathrm{d}v_{-i}.
\label{eq:triple}
\end{align}

Add the revenue to both sides, i.e.\ add
$\int_V f(v)p_i(v)\,\dV$ (and later sum over $i$).
Define
\[
\mathcal{R}_i := \int_V f(v)p_i(v)\,\dV.
\]
Then \eqref{eq:triple} implies
\begin{align}
\mathcal{R}_i
&\le
\mathcal{R}_i
+
\int_{V_{-i}}\int_{V_i}
\int_{[0,H]^m\cup\{\varnothing\}}
\Bigg[
\sum_{j=1}^m v_{ij}\big(x_{ij}(v)-x_{ij}(v_i',v_{-i})\big)
-\big(p_i(v)-p_i(v_i',v_{-i})\big)
\Bigg]\,
\lambda_i^{v_{-i}}(v_i,\mathrm{d}v_i')\,\mathrm{d}v_i\,\mathrm{d}v_{-i}.
\label{eq:addrev}
\end{align}
Expand the right-hand side and collect the payment terms. The coefficient of
$p_i(v)$ in \cref{eq:addrev} is
\[
f(v)
+
\int_{[0,H]^m}\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i)\mathrm{d}u_i
-
\lambda_i^{v_{-i}}(v_i,[0,H]^m\cup\{\varnothing\}).
\]
By flow conservation \cref{eq:flow-cont}, this coefficient equals $0$ for a.e.
$v$. Hence all payment terms cancel, and \cref{eq:addrev} reduces to
\begin{align}
\mathcal{R}_i
&\le
\int_{V_{-i}}\int_{V_i}
\sum_{j=1}^m x_{ij}(v)\,
\Bigg[
v_{ij}
-
\frac{1}{f(v)}
\int_{[0,H]^m}(u_{ij}-v_{ij})\,\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i)
\Bigg]\,
f(v)\,\mathrm{d}v_i\,\mathrm{d}v_{-i}
\nonumber\\
&=
\int_V f(v)\sum_{j=1}^m x_{ij}(v)\,\Phi_{ij}^{\lambda}(v)\,\dV,
\label{eq:rev-to-virt}
\end{align}
where $\Phi^\lambda$ is exactly \eqref{eq:virt-cont}.
Summing \eqref{eq:rev-to-virt} over $i$ gives \eqref{eq:cont-thm24}.

Finally, for each fixed profile $v$, the maximization over feasible $x(\cdot)$
of $\sum_{i,j}x_{ij}(v)\Phi_{ij}^\lambda(v)$ subject to
$x_{ij}(v)\ge 0$ and $\sum_i x_{ij}(v)\le 1$ is separable across items $j$ and
equals $\sum_j \max_i(\Phi_{ij}^\lambda(v))_+$ (a one-line LP argument). This
yields the final displayed bound.
\end{proof}

\paragraph{Interpretation.}
Lemma~\ref{lem:cont-thm24} says: \emph{any} flow-conserving $\lambda$ is a
dual-feasible certificate for the continuous problem, and its induced virtual
values yield an explicit revenue upper bound.


\subsection*{3.\;A coarse-grid dual solution can be lifted to a continuous dual}

We now formalize a coarse discretization (grid) and show how to transform a
coarse dual solution into a continuous flow-conserving $\lambda$ (hence an
upper bound for $\Rev(D)$) \emph{without re-solving any dual}.

\subsubsection*{3.1.\;Grid, cells, and the induced discrete distribution}

Fix, for each bidder $i$ and item $j$, a finite grid
\[
0=t_{ij,0}<t_{ij,1}<\cdots<t_{ij,K_{ij}}=H.
\]
Let the 1D intervals be $I_{ij,k}:=[t_{ij,k-1},t_{ij,k})$ (with the obvious
modification at $k=K_{ij}$ to include $H$).
For bidder $i$, define the cell family
\[
\cC_i:=\Big\{\;C_i(\mathbf{k})=\prod_{j=1}^m I_{ij,k_j}:\ \mathbf{k}\in\prod_{j=1}^m [K_{ij}]\;\Big\}.
\]
For each cell $C_i(\mathbf{k})$, define its \emph{upper corner representative}
\[
\overline{v}_i(C_i(\mathbf{k})) := \big(t_{ij,k_j}\big)_{j=1}^m \in [0,H]^m.
\]
Define the rounding map $\pi_i:[0,H]^m\to \overline{T}_i$ by
$\pi_i(v_i)=\overline{v}_i(C_i)$ where $C_i$ is the unique cell containing
$v_i$, and set $\overline{T}_i:=\{\overline{v}_i(C_i):C_i\in\cC_i\}$.
Let $\pi:V\to \overline{T}:=\prod_i\overline{T}_i$ be $\pi(v)=(\pi_1(v_1),\dots,\pi_n(v_n))$.

The induced discrete (coarse) distribution $\overline{D}$ on $\overline{T}$ is
the law of $\pi(V)$ when $V\sim D$. Its pmf is
\[
\overline{f}(t)=\Pr(\pi(V)=t),
\qquad t\in\overline{T}.
\]
Because $D$ is a product across bidders, $\overline{f}(t)$ factorizes:
\[
\overline{f}(t)=\prod_{i=1}^n \overline{f}_i(t_i),
\qquad
\overline{f}_i(t_i)=\Pr(\pi_i(V_i)=t_i)
=\int_{C_i(t_i)} f_i(v_i)\,\mathrm{d}v_i,
\]
where $C_i(t_i)$ denotes the unique cell with representative $t_i$.

\paragraph{Uniform-mass (optional).}
If we choose the grid so that each cell $C_i\in\cC_i$ has the same probability
mass under $D_i$, then $\overline{f}_i(t_i)$ is constant over $t_i\in\overline{T}_i$,
which simplifies some constants below. None of the arguments require it.

\subsubsection*{3.2.\;Input: a valid coarse dual solution}

Assume we have computed a coarse dual solution in the sense of the document:
for every bidder $i$ and every coarse profile $t_{-i}\in \overline{T}_{-i}$,
we have nonnegative multipliers
\[
\overline{\lambda}_i^{t_{-i}}(t_i,t_i')\ge 0,
\qquad
t_i\in\overline{T}_i,\ \ t_i'\in \overline{T}_i\cup\{\varnothing\},
\]
satisfying the discrete flow conservation constraints (Definition~2.1 in the
document):
\begin{equation}\label{eq:flow-discrete}
\sum_{t_i'\in\overline{T}_i\cup\{\varnothing\}}
\overline{\lambda}_i^{t_{-i}}(t_i,t_i')
\;=\;
\overline{f}(t_i,t_{-i})
+
\sum_{t_i'\in\overline{T}_i}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)
\qquad
\forall t_i\in\overline{T}_i.
\end{equation}
Let $\overline{\Phi}^{\,\overline{\lambda}}$ be the corresponding \emph{discrete}
virtual values (Definition~2.3 in the document):
\begin{equation}\label{eq:virt-discrete}
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)
:=
t_{ij}
-
\frac{1}{\overline{f}(t)}
\sum_{t_i'\in\overline{T}_i}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,\big(t_{i'j}-t_{ij}\big).
\end{equation}
The coarse dual objective value we already know is
\[
\mathrm{UB}_{\mathrm{coarse}}
:=
\sum_{j=1}^m \E_{t\sim \overline{D}}\Big[\,\max_{i\in[n]}\big(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)\big)_+\,\Big]
=
\E_{t\sim\overline{D}}\Big[\sum_{j=1}^m \max_{i}(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t))_+\Big].
\]
By the document's Theorem~2.4, $\mathrm{UB}_{\mathrm{coarse}}$ upper bounds
$\Rev(\overline{D})$ (the optimal revenue in the coarse discrete world).

\subsubsection*{3.3.\;Lifting $\overline{\lambda}$ to a continuous flow-conserving kernel}

We now build a continuous $\lambda$ from $\overline{\lambda}$ by \emph{spreading}
each coarse mass/flow uniformly inside each cell with respect to the
\emph{conditional density}.

\paragraph{Conditional densities inside cells.}
For bidder $i$ define, for almost every $v_i$,
\[
s_i(v_i)
:=
\frac{f_i(v_i)}{\overline{f}_i(\pi_i(v_i))}.
\]
Then for every cell $C_i(t_i)$,
\[
\int_{C_i(t_i)} s_i(v_i)\,\mathrm{d}v_i
=
\frac{1}{\overline{f}_i(t_i)}\int_{C_i(t_i)} f_i(v_i)\,\mathrm{d}v_i
=1,
\]
so $s_i$ is exactly the conditional density of $V_i$ given $\pi_i(V_i)=t_i$.

Similarly, for $v_{-i}$ define
\[
s_{-i}(v_{-i})
:=
\frac{f_{-i}(v_{-i})}{\overline{f}_{-i}(\pi_{-i}(v_{-i}))},
\qquad
\overline{f}_{-i}(t_{-i})=\prod_{k\ne i}\overline{f}_k(t_k).
\]
Then $\int_{C_{-i}(t_{-i})} s_{-i}(v_{-i})\,\mathrm{d}v_{-i}=1$ for each cell of
others.

\paragraph{Definition of the lifted kernel.}
Fix bidder $i$. For almost every $v_{-i}$, let $t_{-i}:=\pi_{-i}(v_{-i})$.
For $v_i\in[0,H]^m$ and a measurable set $A\subseteq [0,H]^m$, define
\begin{equation}\label{eq:lift-kernel}
\lambda_i^{v_{-i}}(v_i,A)
:=
s_{-i}(v_{-i})\,s_i(v_i)\,
\sum_{t_i'\in\overline{T}_i}
\overline{\lambda}_i^{t_{-i}}(\pi_i(v_i),t_i')\,
\int_{A\cap C_i(t_i')} s_i(u_i)\,\mathrm{d}u_i,
\end{equation}
and define the mass to the sink by
\begin{equation}\label{eq:lift-kernel-sink}
\lambda_i^{v_{-i}}(v_i,\{\varnothing\})
:=
s_{-i}(v_{-i})\,s_i(v_i)\,
\overline{\lambda}_i^{t_{-i}}(\pi_i(v_i),\varnothing).
\end{equation}
This specifies a nonnegative kernel on $[0,H]^m\cup\{\varnothing\}$.

\begin{lemma}[Lifted $\lambda$ conserves flow]\label{lem:lift-flow}
Assume $\overline{\lambda}$ satisfies the discrete flow conservation
\eqref{eq:flow-discrete}. Then the lifted kernel $\lambda$ defined by
\eqref{eq:lift-kernel}--\eqref{eq:lift-kernel-sink} satisfies the continuous
flow conservation \eqref{eq:flow-cont} for bidder $i$ (and hence for all bidders).
\end{lemma}

\begin{proof}
Fix bidder $i$. Fix almost every $v_{-i}$ and set $t_{-i}=\pi_{-i}(v_{-i})$.
Fix $v_i$ and set $t_i=\pi_i(v_i)$.

\paragraph{Step 1: compute total outflow from $v_i$.}
By \eqref{eq:lift-kernel} and \eqref{eq:lift-kernel-sink},
\begin{align*}
\lambda_i^{v_{-i}}(v_i,[0,H]^m\cup\{\varnothing\})
&=
\lambda_i^{v_{-i}}(v_i,[0,H]^m)+\lambda_i^{v_{-i}}(v_i,\{\varnothing\})\\
&=
s_{-i}(v_{-i})\,s_i(v_i)\,
\sum_{t_i'\in\overline{T}_i}
\overline{\lambda}_i^{t_{-i}}(t_i,t_i')\,
\underbrace{\int_{C_i(t_i')} s_i(u_i)\,\mathrm{d}u_i}_{=\,1}
\;+\;
s_{-i}(v_{-i})\,s_i(v_i)\,\overline{\lambda}_i^{t_{-i}}(t_i,\varnothing)\\
&=
s_{-i}(v_{-i})\,s_i(v_i)\,
\sum_{t_i'\in\overline{T}_i\cup\{\varnothing\}}
\overline{\lambda}_i^{t_{-i}}(t_i,t_i').
\end{align*}

\paragraph{Step 2: use discrete flow conservation.}
By \eqref{eq:flow-discrete},
\[
\sum_{t_i'\in\overline{T}_i\cup\{\varnothing\}}
\overline{\lambda}_i^{t_{-i}}(t_i,t_i')
=
\overline{f}(t_i,t_{-i})
+
\sum_{t_i'\in\overline{T}_i}\overline{\lambda}_i^{t_{-i}}(t_i',t_i).
\]
Hence
\begin{equation}\label{eq:outflow-expanded}
\lambda_i^{v_{-i}}(v_i,[0,H]^m\cup\{\varnothing\})
=
s_{-i}(v_{-i})\,s_i(v_i)\,\overline{f}(t_i,t_{-i})
+
s_{-i}(v_{-i})\,s_i(v_i)\,\sum_{t_i'\in\overline{T}_i}\overline{\lambda}_i^{t_{-i}}(t_i',t_i).
\end{equation}

\paragraph{Step 3: identify the source term.}
Because $\overline{f}(t_i,t_{-i})=\overline{f}_i(t_i)\overline{f}_{-i}(t_{-i})$,
\[
s_{-i}(v_{-i})\,s_i(v_i)\,\overline{f}(t_i,t_{-i})
=
\frac{f_{-i}(v_{-i})}{\overline{f}_{-i}(t_{-i})}\cdot\frac{f_i(v_i)}{\overline{f}_i(t_i)}\cdot
\overline{f}_i(t_i)\overline{f}_{-i}(t_{-i})
=
f_i(v_i)f_{-i}(v_{-i})
=
f(v_i,v_{-i}).
\]
Thus the first term on the right-hand side of \eqref{eq:outflow-expanded} is
exactly the source inflow $f(v)$ required by \eqref{eq:flow-cont}.

\paragraph{Step 4: compute total inflow into $v_i$.}
We claim
\begin{equation}\label{eq:inflow}
\int_{[0,H]^m}\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i)
=
s_{-i}(v_{-i})\,s_i(v_i)\,\sum_{t_i'\in\overline{T}_i}\overline{\lambda}_i^{t_{-i}}(t_i',t_i).
\end{equation}
To see this, note that by \eqref{eq:lift-kernel}, the measure
$\lambda_i^{v_{-i}}(u_i,\cdot)$ restricted to the cell $C_i(t_i)$ has density
\[
\text{(w.r.t.\ Lebesgue on $C_i(t_i)$)}\qquad
s_{-i}(v_{-i})\,s_i(u_i)\,\overline{\lambda}_i^{t_{-i}}(\pi_i(u_i),t_i)\,s_i(v_i),
\]
because $\int_{A\cap C_i(t_i)} s_i(w)\,\mathrm{d}w$ contributes the factor
$s_i(v_i)$ at the point $v_i$.
Integrating over all $u_i$ and summing over the finitely many source-cells for
$u_i$ gives
\begin{align*}
\int_{[0,H]^m}\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i)
&=
\sum_{t_i'\in\overline{T}_i}\int_{C_i(t_i')} s_{-i}(v_{-i})\,s_i(u_i)\,
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,s_i(v_i)\,\mathrm{d}u_i\\
&=
s_{-i}(v_{-i})\,s_i(v_i)\,\sum_{t_i'\in\overline{T}_i}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)
\underbrace{\int_{C_i(t_i')} s_i(u_i)\,\mathrm{d}u_i}_{=\,1},
\end{align*}
which is exactly \eqref{eq:inflow}.

\paragraph{Step 5: conclude flow conservation.}
Combine \eqref{eq:outflow-expanded} with the identifications in Steps 3 and 4:
\[
\lambda_i^{v_{-i}}(v_i,[0,H]^m\cup\{\varnothing\})
=
f(v_i,v_{-i})
+
\int_{[0,H]^m}\lambda_i^{v_{-i}}(u_i,\mathrm{d}v_i),
\]
which is precisely \eqref{eq:flow-cont} for almost every $(v_i,v_{-i})$.
\end{proof}

\subsubsection*{3.4.\;Therefore, the coarse dual yields a continuous upper bound}

By Lemma~\ref{lem:lift-flow}, the lifted $\lambda$ is flow-conserving, so
Lemma~\ref{lem:cont-thm24} applies.

\begin{theorem}[Continuous upper bound induced by a coarse dual]\label{thm:main-cont-ub}
Let $\overline{\lambda}$ be any coarse dual solution satisfying
\eqref{eq:flow-discrete}, and let $\lambda$ be its lift
\eqref{eq:lift-kernel}--\eqref{eq:lift-kernel-sink}.
Then
\begin{equation}\label{eq:cont-ub}
\Rev(D)
\;\le\;
\int_V f(v)\Big(\sum_{j=1}^m \max_{i\in[n]}(\Phi_{ij}^{\lambda}(v))_+\Big)\,\dV,
\end{equation}
where $\Phi^\lambda$ is given by \eqref{eq:virt-cont}.
\end{theorem}

\paragraph{Remark (explicit formula for $\Phi^\lambda$).}
For computational purposes, one can write $\Phi^\lambda$ in terms of the coarse
data and \emph{cell conditional means}. Define, for each bidder $i$, item $j$,
and coarse representative $t_i\in\overline{T}_i$,
\[
\mu_{ij}(t_i)
:=
\E[V_{ij}\mid \pi_i(V_i)=t_i]
=
\int_{C_i(t_i)} u_{ij}\,s_i(u_i)\,\mathrm{d}u_i.
\]
Then a direct substitution of \eqref{eq:lift-kernel} into \eqref{eq:virt-cont}
gives, for almost every $v$ with $t=\pi(v)$,
\begin{equation}\label{eq:Phi-lifted-explicit}
\Phi_{ij}^{\lambda}(v)
=
v_{ij}
-
\frac{1}{\overline{f}(t)}
\sum_{t_i'\in\overline{T}_i}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,\big(\mu_{ij}(t_i')-v_{ij}\big).
\end{equation}
(Proof: the factors $s_i,s_{-i}$ cancel exactly against $f(v)$, just as in the
discrete derivation of Definition~2.3.)


\subsection*{4.\;A computable bound from the coarse objective value (plus a vanishing grid term)}

Theorem~\ref{thm:main-cont-ub} already answers the question: given the coarse
dual $\overline{\lambda}$, we can lift it to a continuous dual $\lambda$ and
obtain the continuous upper bound \eqref{eq:cont-ub}.

Often one wants an upper bound expressed as:
\[
\text{(coarse dual objective value)} \;+\; \text{(explicit discretization error)}.
\]
We now derive such a bound using the fact that the representatives are
\emph{upper corners} (a ``rounding up'' discretization).

\subsubsection*{4.1.\;Grid geometry and a key nonnegative coefficient}

For a bidder $i$, a cell $C_i(t_i)$, and an item $j$, define the cell's $j$-width
\[
\Delta_{ij}(t_i)
:=
t_{ij}-\inf\{u_{ij}:u_i\in C_i(t_i)\}\ \in[0,H].
\]
Let the worst-case width for item $j$ be
\[
\Delta_j := \max_{i\in[n]}\max_{t_i\in\overline{T}_i}\Delta_{ij}(t_i).
\]
Because $t_i$ is the \emph{upper corner} of its cell,
for all $u_i\in C_i(t_i)$ one has $u_{ij}\le t_{ij}$, hence
\begin{equation}\label{eq:mean-upper}
0\le t_{ij}-\mu_{ij}(t_i)\le \Delta_{ij}(t_i)\le \Delta_j.
\end{equation}

Define the \emph{normalized incoming-flow ratio} (computable from the coarse dual)
\begin{equation}\label{eq:alpha}
\alpha_i(t)
:=
\frac{1}{\overline{f}(t)}
\sum_{t_i'\in\overline{T}_i}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)
\qquad (\ge 0).
\end{equation}

\subsubsection*{4.2.\;Pointwise comparison: lifted continuous virtual values vs.\ coarse virtual values}

Recall the coarse virtual values $\overline{\Phi}^{\,\overline{\lambda}}$ from
\eqref{eq:virt-discrete}. For almost every $v$ and $t=\pi(v)$, compare the lifted
$\Phi^\lambda(v)$ from \eqref{eq:Phi-lifted-explicit} to
$\overline{\Phi}^{\,\overline{\lambda}}(t)$.

\begin{lemma}[One-sided (upper) comparison]\label{lem:one-sided}
For almost every $v\in V$ and $t=\pi(v)$, for every bidder $i$ and item $j$,
\begin{equation}\label{eq:one-sided}
\Phi_{ij}^{\lambda}(v)
\;\le\;
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)
\;+\;
\Delta_j\,\alpha_i(t).
\end{equation}
\end{lemma}

\begin{proof}
Fix $i,j$ and $v$ with $t=\pi(v)$.
Start from the explicit lifted formula \eqref{eq:Phi-lifted-explicit}:
\[
\Phi_{ij}^{\lambda}(v)
=
v_{ij}
-
\frac{1}{\overline{f}(t)}
\sum_{t_i'}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,\big(\mu_{ij}(t_i')-v_{ij}\big).
\]
Expand the term in parentheses:
\[
\mu_{ij}(t_i')-v_{ij} = (\mu_{ij}(t_i')-t_{i'j}) + (t_{i'j}-t_{ij}) + (t_{ij}-v_{ij}).
\]
Substitute and regroup:
\begin{align*}
\Phi_{ij}^{\lambda}(v)
&=
v_{ij}
-
\frac{1}{\overline{f}(t)}
\sum_{t_i'}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(t_{i'j}-t_{ij})
\\
&\quad
-\frac{1}{\overline{f}(t)}
\sum_{t_i'}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(\mu_{ij}(t_i')-t_{i'j})
\\
&\quad
-\frac{1}{\overline{f}(t)}
\sum_{t_i'}
\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(t_{ij}-v_{ij}).
\end{align*}
Now observe:
\begin{itemize}
\item The first line equals $\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)$,
because by \eqref{eq:virt-discrete},
\[
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)
=
t_{ij}
-
\frac{1}{\overline{f}(t)}
\sum_{t_i'}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(t_{i'j}-t_{ij}),
\]
so replacing $t_{ij}$ by $v_{ij}$ changes it by $v_{ij}-t_{ij}\le 0$ (since $t_{ij}$
is the upper endpoint of the interval containing $v_{ij}$).
Formally, write
\[
v_{ij}
-
\frac{1}{\overline{f}(t)}\sum_{t_i'}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)(t_{i'j}-t_{ij})
=
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)\;+\;(v_{ij}-t_{ij})
\;\le\;
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t).
\]
\item The second line is \emph{nonnegative} when moved to the right-hand side,
because $\mu_{ij}(t_i')\le t_{i'j}$ by \eqref{eq:mean-upper}, hence
$\mu_{ij}(t_i')-t_{i'j}\le 0$, and all $\overline{\lambda}\ge 0$.
Thus
\[
-\frac{1}{\overline{f}(t)}
\sum_{t_i'}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(\mu_{ij}(t_i')-t_{i'j})
=
\frac{1}{\overline{f}(t)}
\sum_{t_i'}\overline{\lambda}_i^{t_{-i}}(t_i',t_i)\,(t_{i'j}-\mu_{ij}(t_i'))
\;\le\;
\Delta_j\,\alpha_i(t),
\]
using \eqref{eq:mean-upper} and the definition \eqref{eq:alpha} of $\alpha_i(t)$.
\item The third line is \emph{nonpositive}, since $t_{ij}-v_{ij}\ge 0$ and
$\overline{\lambda}\ge 0$.
\end{itemize}
Combining these three bullets yields
\[
\Phi_{ij}^{\lambda}(v)
\le
\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t) + \Delta_j\,\alpha_i(t),
\]
which is exactly \eqref{eq:one-sided}.
\end{proof}

\subsubsection*{4.3.\;From pointwise comparison to an explicit continuous revenue bound}

Define the random coarse profile $T:=\pi(V)$ when $V\sim D$; then $T\sim\overline{D}$.

\begin{theorem}[Coarse objective $+$ explicit grid error]\label{thm:coarse-plus-error}
Let $\overline{\lambda}$ be any coarse flow-conserving dual solution for
$\overline{D}$, and let $\mathrm{UB}_{\mathrm{coarse}}$ be its (known) coarse dual
objective value.
Then the continuous optimal revenue satisfies
\begin{equation}\label{eq:final-bound}
\Rev(D)
\;\le\;
\mathrm{UB}_{\mathrm{coarse}}
\;+\;
\Big(\sum_{j=1}^m \Delta_j\Big)\cdot
\E_{t\sim\overline{D}}\Big[\max_{i\in[n]}\alpha_i(t)\Big],
\end{equation}
where $\Delta_j$ is the maximum $j$-width of a grid cell and $\alpha_i(t)$ is the
normalized incoming-flow ratio \eqref{eq:alpha} computed from $\overline{\lambda}$.
In particular, the purely worst-case version
\[
\Rev(D)
\;\le\;
\mathrm{UB}_{\mathrm{coarse}}
\;+\;
\Big(\sum_{j=1}^m \Delta_j\Big)\cdot
\max_{t\in\overline{T}}\max_{i\in[n]}\alpha_i(t)
\]
also holds.
\end{theorem}

\begin{proof}
By Theorem~\ref{thm:main-cont-ub},
\[
\Rev(D)\le \int_V f(v)\Big(\sum_{j=1}^m \max_i(\Phi_{ij}^{\lambda}(v))_+\Big)\,\dV.
\]
Fix $v$ and let $t=\pi(v)$. Apply Lemma~\ref{lem:one-sided}:
\[
\Phi_{ij}^{\lambda}(v)\le \overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)+\Delta_j\alpha_i(t).
\]
Since $\Delta_j\alpha_i(t)\ge 0$, we have $(a+b)_+\le a_+ + b$ for $b\ge 0$, hence
\[
\max_i(\Phi_{ij}^{\lambda}(v))_+
\le
\max_i\big(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)+\Delta_j\alpha_i(t)\big)_+
\le
\max_i\big(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)\big)_+
+
\Delta_j\max_i\alpha_i(t).
\]
Sum over $j$:
\[
\sum_{j=1}^m \max_i(\Phi_{ij}^{\lambda}(v))_+
\le
\sum_{j=1}^m \max_i\big(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t)\big)_+
+
\Big(\sum_{j=1}^m\Delta_j\Big)\max_i\alpha_i(t).
\]
Now take expectation over $v\sim D$. The first term depends on $v$ only through
$t=\pi(v)$, so its expectation equals the expectation under $t\sim\overline{D}$:
\[
\E_{v\sim D}\Big[\sum_{j=1}^m \max_i(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(\pi(v)))_+\Big]
=
\E_{t\sim\overline{D}}\Big[\sum_{j=1}^m \max_i(\overline{\Phi}^{\,\overline{\lambda}}_{ij}(t))_+\Big]
=
\mathrm{UB}_{\mathrm{coarse}}.
\]
The second term likewise becomes
\[
\Big(\sum_{j=1}^m\Delta_j\Big)\E_{v\sim D}\big[\max_i\alpha_i(\pi(v))\big]
=
\Big(\sum_{j=1}^m\Delta_j\Big)\E_{t\sim\overline{D}}\big[\max_i\alpha_i(t)\big].
\]
Combining yields \eqref{eq:final-bound}. The worst-case version follows by
$\E[\max_i\alpha_i(t)]\le \max_{t,i}\alpha_i(t)$.
\end{proof}


\subsection*{5.\;How the shifted-copy refinement fits this bound (conceptually)}

The refinement rule (retain all coarse points and add translated copies left,
down, and diagonally) produces a \emph{nested sequence of partitions}
(coarse cells are unions of finer cells). For each fixed coarse dual
$\overline{\lambda}$, the lifting construction in
\eqref{eq:lift-kernel}--\eqref{eq:lift-kernel-sink} produces a \emph{single}
continuous flow-conserving $\lambda$, hence a valid continuous upper bound.

Moreover, if our refinement reduces each coordinate cell-width by (say) a
factor $1/2$ (as in a dyadic refinement), then the geometric quantities
$\Delta_j$ in Theorem~\ref{thm:coarse-plus-error} shrink by the same factor.
Thus, \eqref{eq:final-bound} quantifies how the discretization error in the
upper bound decreases as the grid is refined, \emph{without changing the coarse dual}.
(Any further improvement from refinement would come from recomputing a better
dual on the refined grid, but your question asked explicitly for a bound derived
from the coarse dual.)













\section{Arbitrary Distribution}
Fix any \emph{flow-conserving} coarse dual solution
$\lambda^{\mathrm{C}}=\{\lambda_i^{\mathrm{C},\,w_{-i}}(w_i,w_i')\}$ for $D^{\mathrm{C}}$.
\begin{definition}[Lifted Flow]\label{def:general_lift}
    Define a \emph{lifted} flow $\lambda^{(K)}$ on $G^{(K)}$ as follows.
    
    (1) \textbf{For new fine grid points} $v=(v_i,v_{-i})\in G^{(K)}\setminus G^\mathrm{C}$, the inflow is from $w_i'\in\supp(D^{\mathrm{C}}_i)$:
    \begin{align}
    \label{eq:lift-in_n}
    \lambda_{i}^{(K),\,v_{-i}}(w_i',v_i)
    = \frac{f^{(N)}(v)}{f^{\mathrm{C}}(w)}\;
    \lambda_{i}^{\mathrm{C},\,w_{-i}}\!\bigl(w_i',w_i\bigr).
    \end{align}
    The outflow is to $w_i'\in\supp(D^{\mathrm{C}}_i)$:
    \begin{align}
    \label{eq:lift-out_n}
    \lambda_{i}^{(K),\,v_{-i}}(v_i,w_i')
    = \frac{f^{(K)}(v)}{f^{\mathrm{C}}(w)}\;
    \lambda_{i}^{\mathrm{C},\,w_{-i}}\!\bigl(w_i,w_i'\bigr).
    \end{align}

    Another group of inflow/outflow is as follows: receiving from the super source and sending it to the parent node:
    \begin{align}
    \label{eq:lift-out-balance}
    \lambda_{i}^{(K),\,v_{-i}}(w_i, v_i)=\lambda_{i}^{(K),\,v_{-i}}(v_i,\varnothing)
    = f^{(K)}(v_i).
    \end{align}
    Leave all other flow 0.

    (2) \textbf{For retained coarse grid points} $w=(w_i,v_{-i})\in G^{(K)}$, except for the inflow and outflow we just defined for new fine grid points (Eq.~\ref{eq:lift-in_n} and~\ref{eq:lift-out_n}), it has inflow $f^{(K)}(v_i)$, corresponding to Eq.~\ref{eq:lift-out-balance}.
\end{definition}



\begin{theorem}[Conservation under $N$-fold lift]
\label{lem:flowN}
The $\lambda^{(K)}$ in Definition~\ref{def:general_lift} is flow conserving.
\end{theorem}

\begin{proof}
(1) For new fine grid points $v=(v_i,v_{-i})\in G^{(K)}\setminus G^\mathrm{C}$. Summing the first group of inflow and outflow (Eq.~\ref{eq:lift-in_n} and~\ref{eq:lift-out_n}) over $w_i'$ and subtracting, and then using flow conservation of
$\lambda^{\mathrm{C}}$ at the coarse node $\bigl(w_i,w_{-i}\bigr)$, we obtain
\[
\sum_{w_i'} \lambda_{i}^{(K),\,v_{-i}}(v_i,w_i')
-\sum_{w_i'} \lambda_{i}^{(K),\,v_{-i}}(w_i',v_i)
=
\frac{f^{(K)}(v)}{f^{\mathrm{C}}(w)}\,
\Bigl(f^{\mathrm{C}}(w)\Bigr)
= f^{(K)}(v).
\]
The second group of inflow and outflow (Eq.~\ref{eq:lift-out-balance}) cancels out. So the flow conservation condition is satisfied.

(2) For retained coarse grid points $v=(v_i,v_{-i})\in G^{(K)}$:
\begin{align}
&\underbrace{\lambda_{i}^{(K),\,v_{-i}}(v_i,\varnothing)+\sum_{v_i'} \lambda_{i}^{(K),\,v_{-i}}(v_i,v_i')
-\sum_{v_i'} \lambda_{i}^{(K),\,v_{-i}}(v_i',v_i)}_{\text{Group 1}} - \underbrace{\sum_{v_i'\in S(v_i)\setminus \{v_i\}}\lambda_{i}^{(K),\,v_{-i}}(v_i', v_i)}_{\text{Group 2}}\nonumber\\
=& \lambda_{i}^{(K),\,v_{-i}}(v_i,\varnothing)+\sum_{w_i'}\sum_{v_i'\in S(w')} \lambda_{i}^{(K),\,v_{-i}}(v_i,v_i')
-\sum_{w_i'}\sum_{v_i'\in S(w')} \lambda_{i}^{(K),\,v_{-i}}(v_i',v_i)- \sum_{v_i'\in S(v_i)\setminus \{v_i\}} \frac{f^{(K)}(v_i)}{f^{\mathrm{C}}(w_i)}\nonumber\\
=& \lambda_{i}^{(K),\,v_{-i}}(v_i,\varnothing)+\sum_{w_i'} \lambda_{i}^{\mathrm{C},\,w_{-i}}(w_i,w_i')
-\sum_{w_i'} \lambda_{i}^{\mathrm{C},\,w_{-i}}(w_i',w_i) - (f^{\mathrm{C}}(w_i) - f^{\mathrm{F}}(v_i))\nonumber\\
=&f^{\mathrm{C}}(w_i)-(f^{\mathrm{C}}(w_i) - f^{\mathrm{F}}(v_i))\nonumber\\
=& f^{\mathrm{F}}(v_i) \nonumber
\end{align}


\end{proof}

\begin{theorem}[Dominant virtual values]\label{lem:gapN}
(1) For new fine grid points $v=(v_i,v_{-i})\in G^{(K)}\setminus G^\mathrm{C}$.

Let $v\in G^{(N)}$ and $w:=R(v)\in G^{\mathrm{C}}$. Then for all bidders $i$ and items $j$,
\begin{equation}
\label{eq:gap}
\Phi^{\lambda^{\mathrm{C}}}_{ij}(w)-\Phi^{\lambda^{(N)}}_{ij}(v)
=\Bigl(w_{ij}-v_{ij}\Bigr)\cdot
\left(1+\frac{\sum_{t_i'\in\supp(D^{\mathrm{C}}_i)}\lambda_{i}^{\mathrm{C},\,w_{-i}}(t_i',w_i)}
{f^{\mathrm{C}}(w)}\right)\;\ge 0.
\end{equation}
\end{theorem}

\begin{proof}

(1) For new fine grid points $v=(v_i,v_{-i})\in G^{(K)}\setminus G^\mathrm{C}$.
\[
\Phi^{\lambda^{(K)}}_{ij}(v)
= v_{ij}-\frac{1}{f^{(K)}(v)}\!\sum_{w_i'}\lambda_i^{(K),\,w_{-i}}(w_i',v_i)\,(w'_{ij}-v_{ij})
= v_{ij}-\frac{1}{f^{\mathrm{C}}(w)}\sum_{w_i'}\lambda_i^{\mathrm{C},\,w_{-i}}(w_i',w_i)\,(w'_{ij}-v_{ij}),
\]
Subtracting from
\[
\Phi^{\lambda^{\mathrm{C}}}_{ij}(w)
= w_{ij}-\frac{1}{f^{\mathrm{C}}(w)}\sum_{w_i'}\lambda_i^{\mathrm{C},\,w_{-i}}(w_i',w_i)\,(w'_{ij}-w_{ij}) (\text{TODO: superscript of lambda}?)
\]
yields exactly 
\begin{equation}
\Phi^{\lambda^{\mathrm{C}}}_{ij}(w)-\Phi^{\lambda^{(K)}}_{ij}(v)
=\Bigl(w_{ij}-v_{ij}\Bigr)\cdot
\left(1+\frac{\sum_{w_i'\in\supp(D^{\mathrm{C}}_i)}\lambda_{i}^{\mathrm{C},\,w_{-i}}(w_i',w_i)}
{f^{\mathrm{C}}(w)}\right)\;\ge 0.
\end{equation}

Nonnegativity follows from $w_{ij}\ge v_{ij}$ and $\lambda\ge 0$.


(2) For retained coarse grid points $v=(v_i,v_{-i})\in G^{(K)}$.

\begin{align}
\Phi^{\lambda^{(K)}}_{ij}(v)
&= v_{ij}-\frac{1}{f^{(K)}(v)}\left[\sum_{w_i'}\sum_{v_i'\in S(w_i')}\lambda_i^{(K),\,v_{-i}}(v_i',v_i)\,(v'_{ij}-v_{ij})+\sum_{v_i'\in S(v_i)\setminus\{v_i\} }f^{(K)}(v_i')\right]    \\
&= v_{ij}-\frac{1}{f^{\mathrm{C}}(w)}\sum_{w_i'}\lambda_i^{\mathrm{C},\,w_{-i}}(w_i',v_i)\sum_{v_i'\in S(w_i')}(v'_{ij}-v_{ij})-\frac{1}{f^{(K)}(v)}\sum_{v_i'\in S(v_i)\setminus\{v_i\} }f^{(K)}(v_i')
\end{align}

We have
\[
\Phi^{\lambda^{\mathrm{C}}}_{ij}(w)
= w_{ij}-\frac{1}{f^{\mathrm{C}}(w)}\sum_{w_i'}\lambda_i^{\mathrm{C},\,w_{-i}}(w_i',w_i)\,(w'_{ij}-w_{ij}).
\]

Therefore, 
\begin{align}
    \Phi^{\lambda^{\mathrm{C}}}_{ij}(w) - \Phi^{\lambda^{(K)}}_{ij}(v) &= \frac{1}{f^{\mathrm{C}}(w)}\sum_{w_i'}\lambda_i^{\mathrm{C},\,w_{-i}}(w_i',w_i)\,\sum_{v_i'\in S(w_i')\setminus\{w_i'\}} v_{ij}'+\frac{1}{f^{(K)}(v)}\sum_{v_i'\in S(v_i)\setminus\{v_i\} }f^{(K)}(v_i').\\
    &\ge 0
\end{align}


\end{proof}

